Interpretable Explainability in Facial Emotion Recognition and Gamification for Data Collection

Training facial emotion recognition models requires large sets of data and costly annotation processes. To alleviate this problem, we developed a gamified method of acquiring annotated facial emotion data without an explicit labeling effort by humans. The game, which we named Facegame, challenges the players to imitate a displayed image of a face that portrays a particular basic emotion. Every round played by the player creates new data that consists of a set of facial features and landmarks, already annotated with the emotion label of the target facial expression. Such an approach effectively creates a robust, sustainable, and continuous machine learning training process. We evaluated Facegame with an experiment that revealed several contributions to the field of affective computing. First, the gamified data collection approach allowed us to access a rich variation of facial expressions of each basic emotion due to the natural variations in the players' facial expressions and their expressive abilities. We report improved accuracy when the collected data were used to enrich well-known in-the-wild facial emotion datasets and consecutively used for training facial emotion recognition models. Second, the natural language prescription method used by the Facegame constitutes a novel approach for interpretable explainability that can be applied to any facial emotion recognition model. Finally, we observed significant improvements in the facial emotion perception and expression skills of the players through repeated game play.

==> bib.tex <==
@article{matsumoto2008facial,
  title={Facial expressions of emotion.},
  author={Matsumoto, David and Keltner, Dacher and Shiota, Michelle N and O'Sullivan, Maureen and Frank, Mark},
  year={2008},
  publisher={The Guilford Press}
}
@book{fridlund2014human,
  title={Human facial expression: An evolutionary view},
  author={Fridlund, Alan J},
  year={2014},
  publisher={Academic press}
}
@article{scherer1986vocal,
  title={Vocal affect expression: a review and a model for future research.},
  author={Scherer, Klaus R},
  journal={Psychological bulletin},
  volume={99},
  number={2},
  pages={143},
  year={1986},
  publisher={American Psychological Association}
}
@article{li2020deep,
  title={Deep facial expression recognition: A survey},
  author={Li, Shan and Deng, Weihong},
  journal={IEEE transactions on affective computing},
  year={2020},
  publisher={IEEE}
}
@article{li2018reliable,
  title={Reliable crowdsourcing and deep locality-preserving learning for unconstrained facial expression recognition},
  author={Li, Shan and Deng, Weihong},
  journal={IEEE Transactions on Image Processing},
  volume={28},
  number={1},
  pages={356--370},
  year={2018},
  publisher={IEEE}
}
@article{mollahosseini2017affectnet,
  title={Affectnet: A database for facial expression, valence, and arousal computing in the wild},
  author={Mollahosseini, Ali and Hasani, Behzad and Mahoor, Mohammad H},
  journal={IEEE Transactions on Affective Computing},
  volume={10},
  number={1},
  pages={18--31},
  year={2017},
  publisher={IEEE}
}
@article{zhuexplainable,
  title={Explainable Emotion Recognition for Trustworthy Human-Robot Interaction},
  author={Zhu, Hongbo and Yu, Chuang and Cangelosi, Angelo}
}

@book{picard2000affective,
  title={Affective computing},
  author={Picard, Rosalind W},
  year={2000},
  publisher={MIT press}
}

@article{maithri2022automated,
  title={Automated Emotion Recognition: Current Trends and Future Perspectives},
  author={Maithri, M and Raghavendra, U and Gudigar, Anjan and Samanth, Jyothi and Barua, Prabal Datta and Murugappan, Murugappan and Chakole, Yashas and Acharya, U Rajendra},
  journal={Computer Methods and Programs in Biomedicine},
  pages={106646},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{dalal2005histograms,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  booktitle={2005 IEEE computer society conference on computer vision and pattern recognition (CVPR'05)},
  volume={1},
  pages={886--893},
  year={2005},
  organization={Ieee}
}

@article{cceliktutan2013comparative,
  title={A comparative study of face landmarking techniques},
  author={{\c{C}}eliktutan, Oya and Ulukaya, Sezer and Sankur, B{\"u}lent},
  journal={EURASIP Journal on Image and Video Processing},
  volume={2013},
  number={1},
  pages={1--27},
  year={2013},
  publisher={SpringerOpen}
}

